Ensemble Modeling of Multiple Physical Indicators to Dynamically Phenotype Autism Spectrum Disorder

Early detection of autism, a neurodevelopmental disorder marked by social communication challenges, is crucial for timely intervention. Recent advancements have utilized naturalistic home videos captured via the mobile application GuessWhat. Through interactive games played between children and their guardians, GuessWhat has amassed over 3,000 structured videos from 382 children, both diagnosed with and without Autism Spectrum Disorder (ASD). This collection provides a robust dataset for training computer vision models to detect ASD-related phenotypic markers, including variations in emotional expression, eye contact, and head movements. We have developed a protocol to curate high-quality videos from this dataset, forming a comprehensive training set. Utilizing this set, we trained individual LSTM-based models using eye gaze, head positions, and facial landmarks as input features, achieving test AUCs of 86%, 67%, and 78%, respectively. To boost diagnostic accuracy, we applied late fusion techniques to create ensemble models, improving the overall AUC to 90%. This approach also yielded more equitable results across different genders and age groups. Our methodology offers a significant step forward in the early detection of ASD by potentially reducing the reliance on subjective assessments and making early identification more accessibly and equitable.

==> figures/feature_engineering.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,486); %set diagram left start at 0, and has height of 486

%Flowchart: Alternative Process [id:dp14193802287451818] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (123.4,74.84) .. controls (123.4,68.93) and (128.19,64.14) .. (134.1,64.14) -- (234.88,64.14) .. controls (240.79,64.14) and (245.58,68.93) .. (245.58,74.84) -- (245.58,114.6) .. controls (245.58,120.51) and (240.79,125.3) .. (234.88,125.3) -- (134.1,125.3) .. controls (128.19,125.3) and (123.4,120.51) .. (123.4,114.6) -- cycle ;
%Image [id:dp19974861338898897] 
\draw (567.42,25.81) node  {\includegraphics[width=34.23pt,height=31.12pt]{latex/figures/frame_85.jpg}};
%Image [id:dp24640213526668542] 
\draw (274.29,26.13) node  {\includegraphics[width=39.36pt,height=32.13pt]{latex/figures/frame_28.jpg}};
%Image [id:dp7026706635164364] 
\draw (514.56,25.47) node  {\includegraphics[width=34.52pt,height=31.45pt]{latex/figures/frame_14.jpg}};
%Image [id:dp4844897915351045] 
\draw (672.61,26.27) node  {\includegraphics[width=33.33pt,height=31.86pt]{latex/figures/frame_1.jpg}};
%Image [id:dp3645789114249305] 
\draw (619.85,26.46) node  {\includegraphics[width=33.67pt,height=31.72pt]{latex/figures/frame_2.jpg}};
%Image [id:dp3700255751234671] 
\draw (459.13,25.79) node  {\includegraphics[width=38.12pt,height=31pt]{latex/figures/frame_27.jpg}};
%Image [id:dp9531968794331207] 
\draw (397.55,26.22) node  {\includegraphics[width=39.79pt,height=32.27pt]{latex/figures/frame_26.jpg}};
%Image [id:dp07984098736309186] 
\draw (336.19,26.14) node  {\includegraphics[width=39.03pt,height=32.2pt]{latex/figures/frame_25.jpg}};
%Image [id:dp17861173199673308] 
\draw (152.42,26.32) node  {\includegraphics[width=39.47pt,height=32.42pt]{latex/figures/frame_41.jpg}};
%Image [id:dp891653044866485] 
\draw (213.42,26.68) node  {\includegraphics[width=38.66pt,height=32.96pt]{latex/figures/frame_45.jpg}};
%Image [id:dp5842638446048649] 
\draw (567.99,92.86) node  {\includegraphics[width=34.23pt,height=31.12pt]{latex/figures/frame_85.jpg}};
%Image [id:dp6775867774402147] 
\draw (274.86,93.18) node  {\includegraphics[width=39.36pt,height=32.13pt]{latex/figures/frame_28.jpg}};
%Image [id:dp636748505708826] 
\draw (515.13,92.52) node  {\includegraphics[width=34.52pt,height=31.45pt]{latex/figures/frame_14.jpg}};
%Image [id:dp3014711455226766] 
\draw (673.18,93.32) node  {\includegraphics[width=33.33pt,height=31.86pt]{latex/figures/frame_1.jpg}};
%Image [id:dp921848538249767] 
\draw (620.42,93.51) node  {\includegraphics[width=33.67pt,height=31.72pt]{latex/figures/frame_2.jpg}};
%Image [id:dp08138998692237975] 
\draw (458.94,92.35) node  {\includegraphics[width=39.25pt,height=30.28pt]{latex/figures/frame_27.jpg}};
%Image [id:dp9824702761414907] 
\draw (395.53,92.77) node  {\includegraphics[width=40.98pt,height=31.52pt]{latex/figures/frame_26.jpg}};
%Image [id:dp4067658816774009] 
\draw (336.76,93.19) node  {\includegraphics[width=39.03pt,height=32.2pt]{latex/figures/frame_25.jpg}};
%Image [id:dp09924906994781568] 
\draw (152.99,93.37) node  {\includegraphics[width=39.47pt,height=32.42pt]{latex/figures/frame_41.jpg}};
%Image [id:dp2118922804784673] 
\draw (213.99,93.73) node  {\includegraphics[width=38.66pt,height=32.96pt]{latex/figures/frame_45.jpg}};
%Flowchart: Alternative Process [id:dp6471140528320058] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (422.29,141.52) .. controls (422.29,135.87) and (426.86,131.3) .. (432.51,131.3) -- (519.34,131.3) .. controls (524.99,131.3) and (529.56,135.87) .. (529.56,141.52) -- (529.56,179.47) .. controls (529.56,185.11) and (524.99,189.69) .. (519.34,189.69) -- (432.51,189.69) .. controls (426.86,189.69) and (422.29,185.11) .. (422.29,179.47) -- cycle ;
%Image [id:dp9831679350839253] 
\draw (502.03,161.27) node  {\includegraphics[width=34.47pt,height=29.71pt]{latex/figures/frame_85.jpg}};
%Image [id:dp8573839093515743] 
\draw (201.81,160.47) node  {\includegraphics[width=39.62pt,height=30.67pt]{latex/figures/frame_28.jpg}};
%Image [id:dp9622733400228485] 
\draw (448.81,160.95) node  {\includegraphics[width=34.75pt,height=30.03pt]{latex/figures/frame_14.jpg}};
%Image [id:dp02267624851812644] 
\draw (613.03,161.71) node  {\includegraphics[width=33.56pt,height=30.42pt]{latex/figures/frame_1.jpg}};
%Image [id:dp19668766938401694] 
\draw (559.91,161.89) node  {\includegraphics[width=33.9pt,height=30.28pt]{latex/figures/frame_2.jpg}};
%Image [id:dp6611851001352218] 
\draw (388.15,159.68) node  {\includegraphics[width=39.51pt,height=28.91pt]{latex/figures/frame_27.jpg}};
%Image [id:dp5848627158569499] 
\draw (326.36,160.08) node  {\includegraphics[width=41.25pt,height=30.09pt]{latex/figures/frame_26.jpg}};
%Image [id:dp5359662425761802] 
\draw (264.12,160.49) node  {\includegraphics[width=39.29pt,height=30.74pt]{latex/figures/frame_25.jpg}};
%Image [id:dp17786251114284823] 
\draw (191.58,245.07) node  {\includegraphics[width=40.77pt,height=33.56pt]{latex/figures/frame_28.jpg}};
%Image [id:dp8973410406448141] 
\draw (616.36,244.75) node  {\includegraphics[width=37.56pt,height=32.48pt]{latex/figures/frame_1.jpg}};
%Image [id:dp6534572475178761] 
\draw (556.9,244.94) node  {\includegraphics[width=37.94pt,height=32.33pt]{latex/figures/frame_2.jpg}};
%Image [id:dp18079059418362387] 
\draw (379.54,245.09) node  {\includegraphics[width=40.66pt,height=33.29pt]{latex/figures/frame_27.jpg}};
%Image [id:dp1618265660608844] 
\draw (316.85,244.64) node  {\includegraphics[width=42.45pt,height=32.92pt]{latex/figures/frame_26.jpg}};
%Image [id:dp1577171307382652] 
\draw (253.75,245.08) node  {\includegraphics[width=40.43pt,height=33.63pt]{latex/figures/frame_25.jpg}};
%Shape: Triangle [id:dp6989736534013491] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (300.4,210.7) -- (184,200.7) -- (414.4,200.7) -- cycle ;
%Shape: Triangle [id:dp8520518288990797] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (585.21,210.7) -- (536,200.7) -- (633.4,200.7) -- cycle ;
%Shape: Triangle [id:dp258793092651062] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (599.92,322.38) -- (527.84,312.02) -- (670.52,312.02) -- cycle ;
%Shape: Triangle [id:dp8962766188202751] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (218.6,323.39) -- (146.52,313.03) -- (289.2,313.03) -- cycle ;
%Shape: Triangle [id:dp5996706569480474] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (406.73,323.39) -- (334.64,313.03) -- (477.33,313.03) -- cycle ;

% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (130.07,282.76) -- (217.07,282.76) -- (217.07,305.76) -- (130.07,305.76) -- cycle  ;
\draw (133.07,287.16) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle X^{1} =\left[ x_{1}^{1} ,\ ...,\ x_{d}^{1}\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (221.42,282.76) -- (308.42,282.76) -- (308.42,305.76) -- (221.42,305.76) -- cycle  ;
\draw (224.42,287.16) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle X^{2} =\left[ x_{1}^{2} ,\ ...,\ x_{d}^{2}\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (316.01,282.78) -- (403.01,282.78) -- (403.01,305.78) -- (316.01,305.78) -- cycle  ;
\draw (319.01,287.18) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle X^{3} =\left[ x_{1}^{3} ,\ ...,\ x_{d}^{3}\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (407.68,282.79) -- (494.68,282.79) -- (494.68,305.79) -- (407.68,305.79) -- cycle  ;
\draw (410.68,287.19) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle X^{4} =\left[ x_{1}^{4} ,\ ...,\ x_{d}^{4}\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (509.37,281.78) -- (596.37,281.78) -- (596.37,304.78) -- (509.37,304.78) -- cycle  ;
\draw (512.37,286.18) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle X^{5} =\left[ x_{1}^{5} ,\ ...,\ x_{d}^{5}\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (602.39,281.78) -- (689.39,281.78) -- (689.39,304.78) -- (602.39,304.78) -- cycle  ;
\draw (605.39,286.18) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle X^{6} =\left[ x_{1}^{6} ,\ ...,\ x_{d}^{6}\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (132.1,330.57) -- (306.1,330.57) -- (306.1,356.57) -- (132.1,356.57) -- cycle  ;
\draw (135.1,334.97) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle Z^{1} =\left[\left( x_{1}^{1} +x_{1}^{2}\right) /2,\ ...,\ \left( x_{d}^{1} +x_{d}^{2}\right) /2\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (320.34,330.57) -- (494.34,330.57) -- (494.34,356.57) -- (320.34,356.57) -- cycle  ;
\draw (323.34,334.97) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle Z^{2} =\left[\left( x_{1}^{3} +x_{1}^{4}\right) /2,\ ...,\ \left( x_{d}^{3} +x_{d}^{4}\right) /2\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (512.92,330.43) -- (686.92,330.43) -- (686.92,356.43) -- (512.92,356.43) -- cycle  ;
\draw (515.92,334.83) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle Z^{3} =\left[\left( x_{1}^{5} +x_{1}^{6}\right) /2,\ ...,\ \left( x_{d}^{5} +x_{d}^{6}\right) /2\right]}$};
% Text Node
\draw    (0.2,5.25) -- (120.2,5.25) -- (120.2,39.25) -- (0.2,39.25) -- cycle  ;
\draw (60.2,22.25) node   [align=left] {\begin{minipage}[lt]{79.15pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Raw Input \ (10 fps)}
\end{center}

\end{minipage}};
% Text Node
\draw    (0.2,43.25) -- (120.2,43.25) -- (120.2,132.25) -- (0.2,132.25) -- cycle  ;
\draw (60.2,87.75) node   [align=left] {\begin{minipage}[lt]{79.15pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Truncate unstable frames at the }\\{\footnotesize beginning and the end}
\end{center}

\end{minipage}};
% Text Node
\draw    (1.2,139.25) -- (121.2,139.25) -- (121.2,208.25) -- (1.2,208.25) -- cycle  ;
\draw (61.2,173.75) node   [align=left] {\begin{minipage}[lt]{79.15pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Delete windows }\\{\footnotesize where the camera }\\{\footnotesize is moving}
\end{center}

\end{minipage}};
% Text Node
\draw    (1.2,214.25) -- (121.2,214.25) -- (121.2,285.25) -- (1.2,285.25) -- cycle  ;
\draw (61.2,249.75) node   [align=left] {\begin{minipage}[lt]{79.15pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Concatenate }\\{\footnotesize informative windows of features}
\end{center}

\end{minipage}};
% Text Node
\draw    (1.2,292) -- (120.2,292) -- (120.2,346) -- (1.2,346) -- cycle  ;
\draw (60.7,319) node   [align=left] {\begin{minipage}[lt]{78.47pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Downsampling by }\\{\footnotesize averaging}
\end{center}

\end{minipage}};
% Text Node
\draw    (0.2,351.9) -- (119.2,351.9) -- (119.2,399.9) -- (0.2,399.9) -- cycle  ;
\draw (59.7,375.9) node   [align=left] {\begin{minipage}[lt]{78.47pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Preprocessed Input (5 fps)}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (151.73,368.19) -- (239.73,368.19) -- (239.73,391.19) -- (151.73,391.19) -- cycle  ;
\draw (154.73,372.59) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle Z^{1} =\left[ z_{1}^{1} \ ,\ ...,\ z_{d}^{1}\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (260.18,369.19) -- (348.18,369.19) -- (348.18,392.19) -- (260.18,392.19) -- cycle  ;
\draw (263.18,373.59) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle Z^{2} =\left[ z_{1}^{2} \ ,\ ...,\ z_{d}^{2}\right]}$};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (367.55,369.19) -- (455.55,369.19) -- (455.55,392.19) -- (367.55,392.19) -- cycle  ;
\draw (370.55,373.59) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.62em}{0.74em}\selectfont]  {${\textstyle Z^{3} =\left[ z_{1}^{3} \ ,\ ...,\ z_{d}^{3}\right]}$};


\end{tikzpicture}


==> figures/feature_extraction.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,773); %set diagram left start at 0, and has height of 773

%Down Arrow [id:dp7022736389909261] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (214.47,120.91) -- (217.9,120.91) -- (217.9,110.34) -- (224.78,110.34) -- (224.78,120.91) -- (228.21,120.91) -- (221.34,127.96) -- cycle ;
%Down Arrow [id:dp9955880036882536] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (330.91,120.91) -- (334.34,120.91) -- (334.34,110.34) -- (341.22,110.34) -- (341.22,120.91) -- (344.66,120.91) -- (337.78,127.96) -- cycle ;
%Down Arrow [id:dp8644206004035189] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (487.75,120.91) -- (491.19,120.91) -- (491.19,110.34) -- (498.06,110.34) -- (498.06,120.91) -- (501.5,120.91) -- (494.63,127.96) -- cycle ;
%Down Arrow [id:dp6324937951276093] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (602.96,120.91) -- (606.4,120.91) -- (606.4,110.34) -- (613.27,110.34) -- (613.27,120.91) -- (616.71,120.91) -- (609.84,127.96) -- cycle ;
%Image [id:dp5196186120883854] 
\draw (492.44,73.83) node  {\includegraphics[width=57.29pt,height=43.62pt]{latex/figures/frame0064.jpg}};
%Image [id:dp28667861218205015] 
\draw (220.03,73.47) node  {\includegraphics[width=57.46pt,height=43.74pt]{latex/figures/frame0064.jpg}};
%Image [id:dp39596990017220923] 
\draw (337.14,73.47) node  {\includegraphics[width=57.46pt,height=43.74pt]{latex/figures/frame0060.jpg}};
%Image [id:dp03545269437191245] 
\draw (607.36,73.83) node  {\includegraphics[width=57.29pt,height=43.62pt]{latex/figures/frame0064.jpg}};
%Shape: Rectangle [id:dp17695844576405362] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (163.97,455.66) -- (657.56,455.66) -- (657.56,510.02) -- (163.97,510.02) -- cycle ;
%Shape: Rectangle [id:dp16233736278328248] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (154.14,469.8) -- (651.56,469.8) -- (651.56,528.4) -- (154.14,528.4) -- cycle ;
%Shape: Rectangle [id:dp9579284477041377] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (148.2,483.8) -- (643.56,483.8) -- (643.56,542.4) -- (148.2,542.4) -- cycle ;

% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (172.86,5.66) -- (655.86,5.66) -- (655.86,36.66) -- (172.86,36.66) -- cycle  ;
\draw (414.36,21.16) node   [align=left] {\begin{minipage}[lt]{326.54pt}\setlength\topsep{0pt}
\begin{center}
{\large Video (90 seconds)}
\end{center}

\end{minipage}};
% Text Node
\draw (408.23,68.31) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{...}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (1.47,61.83) -- (136.47,61.83) -- (136.47,92.83) -- (1.47,92.83) -- cycle  ;
\draw (68.97,77.33) node   [align=left] {\begin{minipage}[lt]{89.79pt}\setlength\topsep{0pt}
\begin{center}
Frames (10 fps)
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (1.47,148.56) -- (136.47,148.56) -- (136.47,214.56) -- (1.47,214.56) -- cycle  ;
\draw (68.97,181.56) node   [align=left] {\begin{minipage}[lt]{89.79pt}\setlength\topsep{0pt}
\begin{center}
Eye Gazing\\(AWS Rekognition)
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ]  (174.86,140.81) -- (270.86,140.81) -- (270.86,226.81) -- (174.86,226.81) -- cycle  ;
\draw (222.86,183.81) node   [align=left] {\begin{minipage}[lt]{63.29pt}\setlength\topsep{0pt}
\begin{center}
\textbf{2 features}\\\textit{{\small Yaw,}}\\{\small \textit{Pitch}}\\
\end{center}

\end{minipage}};
% Text Node
\draw (408.01,168.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{...}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (2.52,259.87) -- (136.52,259.87) -- (136.52,325.87) -- (2.52,325.87) -- cycle  ;
\draw (69.52,292.87) node   [align=left] {\begin{minipage}[lt]{89.05pt}\setlength\topsep{0pt}
\begin{center}
Face Landmarks\\(AWS Rekognition)
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (2.61,369.41) -- (138.61,369.41) -- (138.61,438.41) -- (2.61,438.41) -- cycle  ;
\draw (70.61,403.91) node   [align=left] {\begin{minipage}[lt]{90.54pt}\setlength\topsep{0pt}
\begin{center}
Head Landmarks\\(AWS \\Rekognition)
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 233; green, 166; blue, 174 }  ,fill opacity=1 ]  (290.15,140.81) -- (386.15,140.81) -- (386.15,226.81) -- (290.15,226.81) -- cycle  ;
\draw (338.15,183.81) node   [align=left] {\begin{minipage}[lt]{63.2pt}\setlength\topsep{0pt}
\begin{center}
No features Detected
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 254; green, 243; blue, 191 }  ,fill opacity=1 ]  (445.05,140.81) -- (541.05,140.81) -- (541.05,226.81) -- (445.05,226.81) -- cycle  ;
\draw (493.05,183.81) node   [align=left] {\begin{minipage}[lt]{63.2pt}\setlength\topsep{0pt}
\begin{center}

\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 254; green, 243; blue, 191 }  ,fill opacity=1 ]  (561.5,140.81) -- (657.5,140.81) -- (657.5,226.81) -- (561.5,226.81) -- cycle  ;
\draw (609.5,183.81) node   [align=left] {\begin{minipage}[lt]{63.2pt}\setlength\topsep{0pt}
\begin{center}

\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ]  (174.91,253.05) -- (271.91,253.05) -- (271.91,339.05) -- (174.91,339.05) -- cycle  ;
\draw (223.41,296.05) node   [align=left] {\begin{minipage}[lt]{64.04pt}\setlength\topsep{0pt}
\begin{center}
\textbf{60 features}\\{\small \textit{Eyes, Nose, Mouth, Face Shape}}\\
\end{center}

\end{minipage}};
% Text Node
\draw (409.11,284.53) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{...}};
% Text Node
\draw  [fill={rgb, 255:red, 233; green, 166; blue, 174 }  ,fill opacity=1 ]  (290.15,253.05) -- (386.15,253.05) -- (386.15,339.05) -- (290.15,339.05) -- cycle  ;
\draw (338.15,296.05) node   [align=left] {\begin{minipage}[lt]{63.2pt}\setlength\topsep{0pt}
\begin{center}
No features Detected
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 254; green, 243; blue, 191 }  ,fill opacity=1 ]  (445.05,253.05) -- (541.05,253.05) -- (541.05,339.05) -- (445.05,339.05) -- cycle  ;
\draw (493.05,296.05) node   [align=left] {\begin{minipage}[lt]{63.2pt}\setlength\topsep{0pt}
\begin{center}

\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 254; green, 243; blue, 191 }  ,fill opacity=1 ]  (561.5,253.05) -- (657.5,253.05) -- (657.5,339.05) -- (561.5,339.05) -- cycle  ;
\draw (609.5,296.05) node   [align=left] {\begin{minipage}[lt]{63.2pt}\setlength\topsep{0pt}
\begin{center}

\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ]  (173.81,358.8) -- (270.81,358.8) -- (270.81,444.8) -- (173.81,444.8) -- cycle  ;
\draw (222.31,401.8) node   [align=left] {\begin{minipage}[lt]{64.04pt}\setlength\topsep{0pt}
\begin{center}
\textbf{7 features}\\{\small \textit{Bounding Box,}}\\{\small \textit{Head Pose}}\\
\end{center}

\end{minipage}};
% Text Node
\draw (408.01,390.28) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{...}};
% Text Node
\draw  [fill={rgb, 255:red, 233; green, 166; blue, 174 }  ,fill opacity=1 ]  (289.05,358.8) -- (385.05,358.8) -- (385.05,444.8) -- (289.05,444.8) -- cycle  ;
\draw (337.05,401.8) node   [align=left] {\begin{minipage}[lt]{63.2pt}\setlength\topsep{0pt}
\begin{center}
No features Detected 
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 254; green, 243; blue, 191 }  ,fill opacity=1 ]  (443.95,358.8) -- (539.95,358.8) -- (539.95,444.8) -- (443.95,444.8) -- cycle  ;
\draw (491.95,401.8) node   [align=left] {\begin{minipage}[lt]{63.2pt}\setlength\topsep{0pt}
\begin{center}

\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 254; green, 243; blue, 191 }  ,fill opacity=1 ]  (560.4,358.8) -- (656.4,358.8) -- (656.4,444.8) -- (560.4,444.8) -- cycle  ;
\draw (608.4,401.8) node   [align=left] {\begin{minipage}[lt]{63.2pt}\setlength\topsep{0pt}
\begin{center}

\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (2.9,495.06) -- (138.9,495.06) -- (138.9,526.06) -- (2.9,526.06) -- cycle  ;
\draw (70.9,510.56) node   [align=left] {\begin{minipage}[lt]{90.66pt}\setlength\topsep{0pt}
\begin{center}
Output
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 245; green, 239; blue, 166 }  ,fill opacity=1 ]  (152.58,494.9) -- (261.58,494.9) -- (261.58,529.9) -- (152.58,529.9) -- cycle  ;
\draw (207.08,512.4) node   [align=left] {\begin{minipage}[lt]{72pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle \left[ x_{1}^{1} ,\ ...,\ x_{d}^{1}\right]$\\
\end{center}

\end{minipage}};
% Text Node
\draw (387.91,510.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{...}};
% Text Node
\draw  [fill={rgb, 255:red, 233; green, 166; blue, 174 }  ,fill opacity=1 ]  (269.74,494.93) -- (378.74,494.93) -- (378.74,529.93) -- (269.74,529.93) -- cycle  ;
\draw (324.24,512.43) node   [align=left] {\begin{minipage}[lt]{72pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle [ NA,\ ...,NA]$\\
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 254; green, 243; blue, 191 }  ,fill opacity=1 ]  (411.18,494.93) -- (520.18,494.93) -- (520.18,529.93) -- (411.18,529.93) -- cycle  ;
\draw (465.68,512.43) node   [align=left] {\begin{minipage}[lt]{72pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle \left[ x_{1}^{k-1} ,\ ...,\ x_{d}^{k-1}\right]$\\
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 254; green, 243; blue, 191 }  ,fill opacity=1 ]  (527.92,494.93) -- (636.92,494.93) -- (636.92,529.93) -- (527.92,529.93) -- cycle  ;
\draw (582.42,512.43) node   [align=left] {\begin{minipage}[lt]{72pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle \left[ x_{1}^{k} ,\ ...,\ x_{d}^{k}\right]$\\
\end{center}

\end{minipage}};


\end{tikzpicture}


==> figures/filtering_steps.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,358); %set diagram left start at 0, and has height of 358

%Rounded Rect [id:dp3515379037244586] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (10.2,79.92) .. controls (10.2,68.51) and (19.45,59.26) .. (30.86,59.26) -- (92.83,59.26) .. controls (104.24,59.26) and (113.49,68.51) .. (113.49,79.92) -- (113.49,160.2) .. controls (113.49,171.61) and (104.24,180.86) .. (92.83,180.86) -- (30.86,180.86) .. controls (19.45,180.86) and (10.2,171.61) .. (10.2,160.2) -- cycle ;
%Image [id:dp06825064473725484] 
\draw (59.97,141.24) node  {\includegraphics[width=54.34pt,height=42.94pt]{latex/figures/drawing_charade.png}};
%Rounded Rect [id:dp16929281515187844] 
\draw  [fill={rgb, 255:red, 106; green, 165; blue, 238 }  ,fill opacity=1 ] (126.38,52.65) .. controls (126.38,42.62) and (141,20) .. (159.03,20) -- (262.48,20) .. controls (280.51,20) and (295.12,34.62) .. (295.12,52.65) -- (295.12,150.59) .. controls (295.12,168.62) and (280.51,183.23) .. (262.48,183.23) -- (159.03,183.23) .. controls (141,183.23) and (126.38,168.62) .. (126.38,150.59) -- cycle ;
%Rounded Rect [id:dp7668984541463255] 
\draw  [fill={rgb, 255:red, 158; green, 199; blue, 239 }  ,fill opacity=1 ] (307.68,52.65) .. controls (307.68,34.62) and (322.3,20) .. (340.33,20) -- (441.43,20) .. controls (459.46,20) and (474.08,34.62) .. (474.08,52.65) -- (474.08,150.59) .. controls (474.08,168.62) and (459.46,183.23) .. (441.43,183.23) -- (340.33,183.23) .. controls (322.3,183.23) and (307.68,168.62) .. (307.68,150.59) -- cycle ;
%Rounded Rect [id:dp2077557473653513] 
\draw  [fill={rgb, 255:red, 221; green, 235; blue, 255 }  ,fill opacity=1 ] (483.92,52.65) .. controls (483.92,34.62) and (498.54,20) .. (516.57,20) -- (619.55,20) .. controls (637.58,20) and (652.2,34.62) .. (652.2,52.65) -- (652.2,150.59) .. controls (652.2,168.62) and (637.58,183.23) .. (619.55,183.23) -- (516.57,183.23) .. controls (498.54,183.23) and (483.92,168.62) .. (483.92,150.59) -- cycle ;

% Text Node
\draw (10.85,67.25) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {\begin{minipage}[lt]{70.97pt}\setlength\topsep{0pt}
\begin{center}
\textit{\textbf{\underline{Raw Videos}}}\\\textit{\textbf{\underline{(N = 3113)}}}
\end{center}

\end{minipage}};
% Text Node
\draw (161.03,23) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{60.89pt}\setlength\topsep{0pt}
\begin{center}
\textit{\textbf{\underline{{\large Dataset A}}}}\\\textit{{\large \textbf{\underline{(N = 2123}})}}
\end{center}

\end{minipage}};
% Text Node
\draw (347.48,22.72) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {\textit{\textbf{\underline{Dataset B}}}\\\textit{\textbf{\underline{(N = 700}})}};
% Text Node
\draw (528.44,22.9) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {\textit{\textbf{\underline{Dataset C}}}\\\textit{\textbf{\underline{(N = 688)}}}};
% Text Node
\draw (133.49,79.52) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{108.6pt}\setlength\topsep{0pt}
\begin{center}
{\small ASD/NT videos = \textbf{17:1}}\\{\small Male/Female videos = \textbf{3:1}}\\{\small \textbf{245} children with ASD}\\{\small \textbf{43} NT children}
\end{center}

\end{minipage}};
% Text Node
\draw (312.78,79.7) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{108.6pt}\setlength\topsep{0pt}
\begin{center}
{\small ASD/NT videos = \textbf{5:1}}\\{\small Male/Female videos = \textbf{3:1}}\\{\small \textbf{245} children with ASD}\\{\small \textbf{43} NT children}
\end{center}

\end{minipage}};
% Text Node
\draw (489.73,79.7) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{108.6pt}\setlength\topsep{0pt}
\begin{center}
{\small ASD/NT videos = \textbf{5:1}}\\{\small Male/Female videos = \textbf{3:1}}\\{\small \textbf{243} children with ASD}\\{\small \textbf{42} NT children}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (124.75, 209.76) circle [x radius= 60.81, y radius= 59.4]   ;
\draw (82.75,169.76) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{59.02pt}\setlength\topsep{0pt}
\begin{center}
{\small \textit{Video Quality,}}\\{\small \textit{\% of Face,}}\\{\small \textit{Face Size,}}\\{\small \textit{Head Pose}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (300.34, 210.76) circle [x radius= 54.45, y radius= 59.4]   ;
\draw (262.84,170.76) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{52.56pt}\setlength\topsep{0pt}
\begin{center}
{\small \textit{Balance }}\\{\small \textit{ASD/NT,}}\\{\small \textit{Balance }}\\{\small \textit{Super-users}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (480.51, 210.57) circle [x radius= 84.85, y radius= 59.4]   ;
\draw (421.51,170.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{81.83pt}\setlength\topsep{0pt}
\begin{center}
{\small Discard videos}\\{\small with unsufficient }\\{\small features after}\\{\small feature engineering}
\end{center}

\end{minipage}};


\end{tikzpicture}


==> figures/superusers_plot.tex <==


\begin{tikzpicture}

\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{darkorange25512714}{RGB}{255,127,14}

\begin{axis}[
    tick align=outside,
    tick pos=left,
    title={Number of Videos per Child},
    x grid style={white!69.0196078431373!black},
    xlabel={Number of Videos},
    xmin=-3.45, xmax=94.45,
    xtick style={color=black},
    y grid style={white!69.0196078431373!black},
    ylabel={Count (log scale)},
    ymin=0, ymax=172.2,
    ymode=log, % If you need log scale
    ytick style={color=black}
]

% ASD Histogram Data
\addplot[
    ybar,
    fill=steelblue31119180,
    draw=none,
    area legend
] table[row sep=crcr]{
    x y\\
    1 164\\
    5.45 22\\
    9.9 14\\
    14.35 12\\
    18.8 8\\
    23.25 5\\
    27.7 9\\
    32.15 2\\
    36.6 3\\
    41.05 1\\
    45.5 0\\
    49.95 1\\
    54.4 1\\
    58.85 1\\
    63.3 0\\
    67.75 0\\
    72.2 0\\
    76.65 0\\
    81.1 0\\
    85.55 1\\
    90 1\\
};
\addlegendentry{ASD}

% NT Histogram Data
\addplot[
    ybar,
    fill=darkorange25512714,
    draw=none,
    area legend
] table[row sep=crcr]{
    x y\\
    1 31\\
    2.2 4\\
    3.4 4\\
    4.6 0\\
    5.8 1\\
    7 1\\
    8.2 0\\
    9.4 1\\
    10.6 0\\
    11.8 0\\
    13 0\\
    14.2 0\\
    15.4 0\\
    16.6 0\\
    17.8 0\\
    19 0\\
    20.2 0\\
    21.4 0\\
    22.6 0\\
    23.8 1\\
};
\addlegendentry{NT}

\end{axis}
\end{tikzpicture}


==> figures/upset_plot.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,343); %set diagram left start at 0, and has height of 343

%Shape: Rectangle [id:dp9894179232387863] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.84 ] (257,229.6) -- (492.2,229.6) -- (492.2,250.6) -- (257,250.6) -- cycle ;
%Shape: Rectangle [id:dp2309087929281457] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.84 ] (257,254.6) -- (492.2,254.6) -- (492.2,275.6) -- (257,275.6) -- cycle ;
%Shape: Rectangle [id:dp1036549643029765] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.84 ] (257,279.6) -- (492.2,279.6) -- (492.2,300.6) -- (257,300.6) -- cycle ;
%Shape: Circle [id:dp1429985205581492] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (440,240.1) .. controls (440,235.63) and (443.63,232) .. (448.1,232) .. controls (452.57,232) and (456.2,235.63) .. (456.2,240.1) .. controls (456.2,244.57) and (452.57,248.2) .. (448.1,248.2) .. controls (443.63,248.2) and (440,244.57) .. (440,240.1) -- cycle ;
%Shape: Circle [id:dp28634105404968957] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (440,266.1) .. controls (440,261.63) and (443.63,258) .. (448.1,258) .. controls (452.57,258) and (456.2,261.63) .. (456.2,266.1) .. controls (456.2,270.57) and (452.57,274.2) .. (448.1,274.2) .. controls (443.63,274.2) and (440,270.57) .. (440,266.1) -- cycle ;
%Shape: Circle [id:dp32071915259570094] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (440,291.1) .. controls (440,286.63) and (443.63,283) .. (448.1,283) .. controls (452.57,283) and (456.2,286.63) .. (456.2,291.1) .. controls (456.2,295.57) and (452.57,299.2) .. (448.1,299.2) .. controls (443.63,299.2) and (440,295.57) .. (440,291.1) -- cycle ;
%Shape: Circle [id:dp8404177187232158] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (327,239.9) .. controls (327,235.43) and (330.63,231.8) .. (335.1,231.8) .. controls (339.57,231.8) and (343.2,235.43) .. (343.2,239.9) .. controls (343.2,244.37) and (339.57,248) .. (335.1,248) .. controls (330.63,248) and (327,244.37) .. (327,239.9) -- cycle ;
%Shape: Circle [id:dp7375098736702854] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (327,265.9) .. controls (327,261.43) and (330.63,257.8) .. (335.1,257.8) .. controls (339.57,257.8) and (343.2,261.43) .. (343.2,265.9) .. controls (343.2,270.37) and (339.57,274) .. (335.1,274) .. controls (330.63,274) and (327,270.37) .. (327,265.9) -- cycle ;
%Shape: Circle [id:dp21504406486561245] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (327,290.9) .. controls (327,286.43) and (330.63,282.8) .. (335.1,282.8) .. controls (339.57,282.8) and (343.2,286.43) .. (343.2,290.9) .. controls (343.2,295.37) and (339.57,299) .. (335.1,299) .. controls (330.63,299) and (327,295.37) .. (327,290.9) -- cycle ;
%Straight Lines [id:da20685645900923322] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=2.25]    (448.1,240.1) -- (448.1,291.1) ;
%Straight Lines [id:da05629826223635459] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=2.25]    (335.1,265.9) -- (335.1,290.9) ;
%Shape: Rectangle [id:dp12284614422218265] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (106.2,279.6) -- (211.2,279.6) -- (211.2,300.6) -- (106.2,300.6) -- cycle ;
%Shape: Rectangle [id:dp5623746658321371] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (106.2,254.6) -- (211.2,254.6) -- (211.2,275.6) -- (106.2,275.6) -- cycle ;
%Shape: Rectangle [id:dp626513623120299] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (140.2,229.6) -- (211.2,229.6) -- (211.2,250.6) -- (140.2,250.6) -- cycle ;
%Straight Lines [id:da8173794740199245] 
\draw    (210.2,308.6) -- (166.2,308.6) -- (137.2,308.6) -- (101.2,308.6) (195.2,312.6) -- (195.2,304.6)(180.2,312.6) -- (180.2,304.6)(165.2,312.6) -- (165.2,304.6)(150.2,312.6) -- (150.2,304.6)(135.2,312.6) -- (135.2,304.6)(120.2,312.6) -- (120.2,304.6)(105.2,312.6) -- (105.2,304.6) ;
%Shape: Rectangle [id:dp44286697722553425] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (291.2,142.6) -- (378.2,142.6) -- (378.2,208.6) -- (291.2,208.6) -- cycle ;
%Shape: Rectangle [id:dp14240754815153833] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (401.2,76.6) -- (488.2,76.6) -- (488.2,208.6) -- (401.2,208.6) -- cycle ;
%Straight Lines [id:da53489645114401] 
\draw    (281.2,208.6) -- (500.2,208.6) ;
%Shape: Boxed Line [id:dp9788142899292376] 
\draw    (281.2,208.6) -- (281.2,136.1) -- (281.2,116.14) -- (281.2,65.6) ;
\draw [shift={(281.2,63.6)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8806182479207099] 
\draw    (281.2,61.1) -- (281.2,208.6) (286.2,91.1) -- (276.2,91.1)(286.2,121.1) -- (276.2,121.1)(286.2,151.1) -- (276.2,151.1)(286.2,181.1) -- (276.2,181.1) ;

% Text Node
\draw (216,231) node [anchor=north west][inner sep=0.75pt]   [align=left] {Eye};
% Text Node
\draw (216,257) node [anchor=north west][inner sep=0.75pt]   [align=left] {Head};
% Text Node
\draw (216,283) node [anchor=north west][inner sep=0.75pt]   [align=left] {Face};
% Text Node
\draw (113,312) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny 600 \ \ \ \ \ \ \ \ \ \ \ \ 400 \ \ \ \ \ \ \ \ \ \ 200}};
% Text Node
\draw (116,231) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize 463}};
% Text Node
\draw (82,257) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize 689}};
% Text Node
\draw (83,283) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize 689}};
% Text Node
\draw (254,37) node [anchor=north west][inner sep=0.75pt]   [align=left] {Upset Plot of Video Keys Intersection};
% Text Node
\draw (254,85) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small 400}};
% Text Node
\draw (255,114) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small 300}};
% Text Node
\draw (255,144) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small 200}};
% Text Node
\draw (255,174) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small 100}};
% Text Node
\draw (323,124) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small 226}};
% Text Node
\draw (433,58) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small 463}};


\end{tikzpicture}


==> latex/figures/upset_plot.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,343); %set diagram left start at 0, and has height of 343

%Shape: Rectangle [id:dp9894179232387863] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.84 ] (257,229.6) -- (492.2,229.6) -- (492.2,250.6) -- (257,250.6) -- cycle ;
%Shape: Rectangle [id:dp2309087929281457] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.84 ] (257,254.6) -- (492.2,254.6) -- (492.2,275.6) -- (257,275.6) -- cycle ;
%Shape: Rectangle [id:dp1036549643029765] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.84 ] (257,279.6) -- (492.2,279.6) -- (492.2,300.6) -- (257,300.6) -- cycle ;
%Shape: Circle [id:dp1429985205581492] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (440,240.1) .. controls (440,235.63) and (443.63,232) .. (448.1,232) .. controls (452.57,232) and (456.2,235.63) .. (456.2,240.1) .. controls (456.2,244.57) and (452.57,248.2) .. (448.1,248.2) .. controls (443.63,248.2) and (440,244.57) .. (440,240.1) -- cycle ;
%Shape: Circle [id:dp28634105404968957] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (440,266.1) .. controls (440,261.63) and (443.63,258) .. (448.1,258) .. controls (452.57,258) and (456.2,261.63) .. (456.2,266.1) .. controls (456.2,270.57) and (452.57,274.2) .. (448.1,274.2) .. controls (443.63,274.2) and (440,270.57) .. (440,266.1) -- cycle ;
%Shape: Circle [id:dp32071915259570094] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (440,291.1) .. controls (440,286.63) and (443.63,283) .. (448.1,283) .. controls (452.57,283) and (456.2,286.63) .. (456.2,291.1) .. controls (456.2,295.57) and (452.57,299.2) .. (448.1,299.2) .. controls (443.63,299.2) and (440,295.57) .. (440,291.1) -- cycle ;
%Shape: Circle [id:dp8404177187232158] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (327,239.9) .. controls (327,235.43) and (330.63,231.8) .. (335.1,231.8) .. controls (339.57,231.8) and (343.2,235.43) .. (343.2,239.9) .. controls (343.2,244.37) and (339.57,248) .. (335.1,248) .. controls (330.63,248) and (327,244.37) .. (327,239.9) -- cycle ;
%Shape: Circle [id:dp7375098736702854] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (327,265.9) .. controls (327,261.43) and (330.63,257.8) .. (335.1,257.8) .. controls (339.57,257.8) and (343.2,261.43) .. (343.2,265.9) .. controls (343.2,270.37) and (339.57,274) .. (335.1,274) .. controls (330.63,274) and (327,270.37) .. (327,265.9) -- cycle ;
%Shape: Circle [id:dp21504406486561245] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (327,290.9) .. controls (327,286.43) and (330.63,282.8) .. (335.1,282.8) .. controls (339.57,282.8) and (343.2,286.43) .. (343.2,290.9) .. controls (343.2,295.37) and (339.57,299) .. (335.1,299) .. controls (330.63,299) and (327,295.37) .. (327,290.9) -- cycle ;
%Straight Lines [id:da20685645900923322] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=2.25]    (448.1,240.1) -- (448.1,291.1) ;
%Straight Lines [id:da05629826223635459] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=2.25]    (335.1,265.9) -- (335.1,290.9) ;
%Shape: Rectangle [id:dp12284614422218265] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (106.2,279.6) -- (211.2,279.6) -- (211.2,300.6) -- (106.2,300.6) -- cycle ;
%Shape: Rectangle [id:dp5623746658321371] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (106.2,254.6) -- (211.2,254.6) -- (211.2,275.6) -- (106.2,275.6) -- cycle ;
%Shape: Rectangle [id:dp626513623120299] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (140.2,229.6) -- (211.2,229.6) -- (211.2,250.6) -- (140.2,250.6) -- cycle ;
%Straight Lines [id:da8173794740199245] 
\draw    (210.2,308.6) -- (166.2,308.6) -- (137.2,308.6) -- (101.2,308.6) (195.2,312.6) -- (195.2,304.6)(180.2,312.6) -- (180.2,304.6)(165.2,312.6) -- (165.2,304.6)(150.2,312.6) -- (150.2,304.6)(135.2,312.6) -- (135.2,304.6)(120.2,312.6) -- (120.2,304.6)(105.2,312.6) -- (105.2,304.6) ;
%Shape: Rectangle [id:dp44286697722553425] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (291.2,142.6) -- (378.2,142.6) -- (378.2,208.6) -- (291.2,208.6) -- cycle ;
%Shape: Rectangle [id:dp14240754815153833] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (401.2,76.6) -- (488.2,76.6) -- (488.2,208.6) -- (401.2,208.6) -- cycle ;
%Straight Lines [id:da53489645114401] 
\draw    (281.2,208.6) -- (500.2,208.6) ;
%Shape: Boxed Line [id:dp9788142899292376] 
\draw    (281.2,208.6) -- (281.2,136.1) -- (281.2,116.14) -- (281.2,65.6) ;
\draw [shift={(281.2,63.6)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8806182479207099] 
\draw    (281.2,61.1) -- (281.2,208.6) (286.2,91.1) -- (276.2,91.1)(286.2,121.1) -- (276.2,121.1)(286.2,151.1) -- (276.2,151.1)(286.2,181.1) -- (276.2,181.1) ;

% Text Node
\draw (216,231) node [anchor=north west][inner sep=0.75pt]   [align=left] {Eye};
% Text Node
\draw (216,257) node [anchor=north west][inner sep=0.75pt]   [align=left] {Head};
% Text Node
\draw (216,283) node [anchor=north west][inner sep=0.75pt]   [align=left] {Face};
% Text Node
\draw (113,312) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny 600 \ \ \ \ \ \ \ \ \ \ \ \ 400 \ \ \ \ \ \ \ \ \ \ 200}};
% Text Node
\draw (116,231) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize 463}};
% Text Node
\draw (82,257) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize 689}};
% Text Node
\draw (83,283) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize 689}};
% Text Node
\draw (254,37) node [anchor=north west][inner sep=0.75pt]   [align=left] {Upset Plot of Video Keys Intersection};
% Text Node
\draw (254,85) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small 400}};
% Text Node
\draw (255,114) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small 300}};
% Text Node
\draw (255,144) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small 200}};
% Text Node
\draw (255,174) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small 100}};
% Text Node
\draw (323,124) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small 226}};
% Text Node
\draw (433,58) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small 463}};


\end{tikzpicture}


==> latex/fusion.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,584); %set diagram left start at 0, and has height of 584

%Bend Up Arrow [id:dp5573481551848436] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (300.57,139.48) -- (455.78,139.48) -- (455.78,130.18) -- (451.13,130.18) -- (460.43,117.78) -- (469.73,130.18) -- (465.08,130.18) -- (465.08,148.78) -- (300.57,148.78) -- cycle ;
%Bend Up Arrow [id:dp33236104640148323] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (300.45,39.48) -- (456.49,39.48) -- (456.49,48.18) -- (452.14,48.18) -- (460.84,59.78) -- (469.54,48.18) -- (465.19,48.18) -- (465.19,30.78) -- (300.45,30.78) -- cycle ;
%Right Arrow [id:dp7092644536672368] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (300.45,81.72) -- (420.3,81.72) -- (420.3,76.78) -- (439.88,86.67) -- (420.3,96.56) -- (420.3,91.61) -- (300.45,91.61) -- cycle ;
%Right Arrow [id:dp6469191605367872] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (299.95,256.29) -- (419.94,256.29) -- (419.94,251.16) -- (439.54,261.42) -- (419.94,271.67) -- (419.94,266.54) -- (299.95,266.54) -- cycle ;
%Right Arrow [id:dp34467362638077526] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (300.85,203.91) -- (422.73,203.91) -- (422.73,198.78) -- (442.64,209.03) -- (422.73,219.28) -- (422.73,214.16) -- (300.85,214.16) -- cycle ;
%Right Arrow [id:dp8044476229111577] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (300.85,306.4) -- (422.73,306.4) -- (422.73,301.28) -- (442.64,311.53) -- (422.73,321.78) -- (422.73,316.65) -- (300.85,316.65) -- cycle ;
%Right Arrow [id:dp9797618284662994] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (500.15,260.29) -- (548.84,260.29) -- (548.84,255.16) -- (575.12,265.42) -- (548.84,275.67) -- (548.84,270.54) -- (500.15,270.54) -- cycle ;
%Straight Lines [id:da12863414192269196] 
\draw [line width=1.5]    (131.09,13.34) -- (131.45,353.56) ;
%Right Arrow [id:dp8037210703107915] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (499.44,460.72) -- (548.12,460.72) -- (548.12,455.59) -- (574.41,465.84) -- (548.12,476.09) -- (548.12,470.97) -- (499.44,470.97) -- cycle ;
%Right Arrow [id:dp39876049375085776] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (306.04,460.72) -- (426.04,460.72) -- (426.04,455.59) -- (445.64,465.84) -- (426.04,476.09) -- (426.04,470.97) -- (306.04,470.97) -- cycle ;
%Right Arrow [id:dp4167128510169149] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (306.95,405.33) -- (428.83,405.33) -- (428.83,400.21) -- (448.73,410.46) -- (428.83,420.71) -- (428.83,415.58) -- (306.95,415.58) -- cycle ;
%Right Arrow [id:dp6477951600345084] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (304.95,520.83) -- (426.83,520.83) -- (426.83,515.7) -- (446.73,525.95) -- (426.83,536.21) -- (426.83,531.08) -- (304.95,531.08) -- cycle ;
%Straight Lines [id:da7643014252270415] 
\draw [line width=1.5]    (132.19,384.98) -- (133.28,564.32) ;

% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (139.09,22.88) -- (247.09,22.88) -- (247.09,53.88) -- (139.09,53.88) -- cycle  ;
\draw (193.09,38.38) node   [align=left] {\begin{minipage}[lt]{71.59pt}\setlength\topsep{0pt}
\begin{center}
Eye Model
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (20.21,190.76) -- (118.21,190.76) -- (118.21,241.76) -- (20.21,241.76) -- cycle  ;
\draw (69.21,216.26) node   [align=left] {\begin{minipage}[lt]{64.8pt}\setlength\topsep{0pt}
\begin{center}
Late \\Fusion
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (139.25,74.88) -- (248.25,74.88) -- (248.25,107.88) -- (139.25,107.88) -- cycle  ;
\draw (193.75,91.38) node   [align=left] {\begin{minipage}[lt]{71.67pt}\setlength\topsep{0pt}
\begin{center}
Face Model
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (141.09,125.88) -- (248.09,125.88) -- (248.09,158.88) -- (141.09,158.88) -- cycle  ;
\draw (194.59,142.38) node   [align=left] {\begin{minipage}[lt]{70.91pt}\setlength\topsep{0pt}
\begin{center}
Head Model
\end{center}

\end{minipage}};
% Text Node
\draw (259.8,28) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle O_{1}$};
% Text Node
\draw (258.8,80) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle O_{2}$};
% Text Node
\draw (260.9,135) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle O_{3}$};
% Text Node
\draw  [fill={rgb, 255:red, 179; green, 211; blue, 248 }  ,fill opacity=1 ]  (443.11,63) -- (629.11,63) -- (629.11,111) -- (443.11,111) -- cycle  ;
\draw (446.11,67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle O_{final} =\ \frac{( O_{1} +O_{2} +O_{3})}{3}$};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (452.44,187.34) -- (486.35,187.34) -- (486.35,344.48) -- (452.44,344.48) -- cycle  ;
\draw (469.39,265.91) node  [rotate=-269.66,xslant=0] [align=left] {\begin{minipage}[lt]{104.73pt}\setlength\topsep{0pt}
\begin{center}
Linear Layer
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 179; green, 211; blue, 248 }  ,fill opacity=1 ]  (591.11,247) -- (638.11,247) -- (638.11,273) -- (591.11,273) -- cycle  ;
\draw (594.11,251) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle O_{final}$};
% Text Node
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ]  (274.64, 15.11) circle [x radius= 30.41, y radius= 14.14]   ;
\draw (254.14,7.11) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{29.94pt}\setlength\topsep{0pt}
\begin{center}
\textit{Logits}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (6.95,444.08) -- (117.95,444.08) -- (117.95,497.08) -- (6.95,497.08) -- cycle  ;
\draw (62.45,470.58) node   [align=left] {\begin{minipage}[lt]{73.49pt}\setlength\topsep{0pt}
\begin{center}
Intermediate\\Fusion
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 179; green, 211; blue, 248 }  ,fill opacity=1 ]  (581.4,452.43) -- (628.4,452.43) -- (628.4,478.43) -- (581.4,478.43) -- cycle  ;
\draw (584.4,456.43) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle O_{final}$};
% Text Node
\draw (260.9,404.43) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle H_{1}$};
% Text Node
\draw (260.9,458.43) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle H_{2}$};
% Text Node
\draw (260.99,511.43) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle H_{3}$};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (453.96,390.77) -- (487.87,390.77) -- (487.87,547.91) -- (453.96,547.91) -- cycle  ;
\draw (470.92,469.34) node  [rotate=-269.66,xslant=0] [align=left] {\begin{minipage}[lt]{104.73pt}\setlength\topsep{0pt}
\begin{center}
MLP
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ]  (276.83, 373.93) circle [x radius= 61.65, y radius= 29.27]   ;
\draw (234.41,355.23) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.26] [align=left] {\begin{minipage}[lt]{59.98pt}\setlength\topsep{0pt}
\begin{center}
\textit{Final Hidden}\\\textit{Dimensions }
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (139.09,196.76) -- (247.09,196.76) -- (247.09,227.76) -- (139.09,227.76) -- cycle  ;
\draw (193.09,212.26) node   [align=left] {\begin{minipage}[lt]{71.59pt}\setlength\topsep{0pt}
\begin{center}
Eye Model
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (139.25,248.76) -- (248.25,248.76) -- (248.25,281.76) -- (139.25,281.76) -- cycle  ;
\draw (193.75,265.26) node   [align=left] {\begin{minipage}[lt]{71.67pt}\setlength\topsep{0pt}
\begin{center}
Face Model
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (141.09,299.76) -- (248.09,299.76) -- (248.09,332.76) -- (141.09,332.76) -- cycle  ;
\draw (194.59,316.26) node   [align=left] {\begin{minipage}[lt]{70.91pt}\setlength\topsep{0pt}
\begin{center}
Head Model
\end{center}

\end{minipage}};
% Text Node
\draw (259.8,201.89) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle O_{1}$};
% Text Node
\draw (258.8,253.89) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle O_{2}$};
% Text Node
\draw (260.9,308.89) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle O_{3}$};
% Text Node
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ]  (274.64, 189) circle [x radius= 30.41, y radius= 14.14]   ;
\draw (254.14,181) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{29.94pt}\setlength\topsep{0pt}
\begin{center}
\textit{Logits}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (142.09,400.76) -- (250.09,400.76) -- (250.09,431.76) -- (142.09,431.76) -- cycle  ;
\draw (196.09,416.26) node   [align=left] {\begin{minipage}[lt]{71.59pt}\setlength\topsep{0pt}
\begin{center}
Eye Model
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (142.25,452.76) -- (251.25,452.76) -- (251.25,485.76) -- (142.25,485.76) -- cycle  ;
\draw (196.75,469.26) node   [align=left] {\begin{minipage}[lt]{71.67pt}\setlength\topsep{0pt}
\begin{center}
Face Model
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 203; green, 199; blue, 199 }  ,fill opacity=1 ]  (144.09,503.76) -- (251.09,503.76) -- (251.09,536.76) -- (144.09,536.76) -- cycle  ;
\draw (197.59,520.26) node   [align=left] {\begin{minipage}[lt]{70.91pt}\setlength\topsep{0pt}
\begin{center}
Head Model
\end{center}

\end{minipage}};


\end{tikzpicture}


==> latex/normalization.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,513); %set diagram left start at 0, and has height of 513

%Image [id:dp9774434845672941] 
\draw (328.5,215.77) node  {\includegraphics[width=495.59pt,height=326.25pt]{normalization.png}};
%Shape: Rectangle [id:dp6043638253100345] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]  (15.89,116) -- (648.89,116) -- (648.89,193.05) -- (15.89,193.05) -- cycle ;
%Shape: Rectangle [id:dp8770490699096793] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]  (15.89,310.05) -- (647.89,310.05) -- (647.89,385.05) -- (15.89,385.05) -- cycle ;
%Straight Lines [id:da9489144251331829] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (15.89,46.05) -- (102.89,46.05) ;
%Straight Lines [id:da882870634268138] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (274.89,45.05) -- (369.89,45.05) ;
%Straight Lines [id:da8987606928656555] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (15.89,46.05) -- (15.89,68.05) ;
%Straight Lines [id:da4809556927722838] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (369.89,45.05) -- (369.89,67.05) ;
%Straight Lines [id:da9096577539786723] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (381.89,46.05) -- (381.89,68.05) ;
%Straight Lines [id:da24062391895858992] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (650.89,45.05) -- (650.89,67.05) ;
%Straight Lines [id:da038231037433362314] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (381.89,46.05) -- (408.89,46.05) ;
%Straight Lines [id:da3731185255515528] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (623.89,45.05) -- (650.89,45.05) ;
%Flowchart: Merge [id:dp022637191303015003] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (17.89,239) -- (646.89,239) -- (332.39,260.38) -- cycle ;

% Text Node
\draw (109,37) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{pcr}\selectfont \textcolor[rgb]{0.25,0.46,0.02}{\textit{\textbf{ranges from 0 to 1}}}}};
% Text Node
\draw (413,37) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{pcr}\selectfont \textit{\textbf{\textcolor[rgb]{0.25,0.46,0.02}{ranges from -180 to 180}}}}};


\end{tikzpicture}


==> latex/plot.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Publication Date},
xmin=14410, xmax=19830,
xtick style={color=black},
xtick={13879,14610,15340,16071,16801,17532,18262,18993,19723},
xticklabels={2008,2010,2012,2014,2016,2018,2020,2022,2024},
y grid style={darkgray176},
ylabel={Training compute (Terraflop)},
ymin=36.059848328477, ymax=76289838352633.9,
ymode=log,
ytick style={color=black},
ytick={0.1,10,1000,100000,10000000,1000000000,100000000000,10000000000000,1e+15,1e+17},
yticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{9}}\),
  \(\displaystyle {10^{11}}\),
  \(\displaystyle {10^{13}}\),
  \(\displaystyle {10^{15}}\),
  \(\displaystyle {10^{17}}\)
}
]
\addplot [draw=black, fill=black, mark=*, only marks]
table{%
x  y
14410 1000
14669 131
14742 350
14878 3410
14878 61400
15383 3730
15494 6040
15613 470000
15706 2300
15970 137000
15994 38900
16021 532000
16044 1340930
16059 475.2
16231 518000
16239 6110000
16314 1560000
16317 8524000
16323 7300000
16426 60500
16472 24000000
16593 1560000
16687 380000000
16777 26000000
16779 12100000
16827 1900000000
16973 61492.9
17003 145411
17003 96940.8
17070 6900000000
17081 44000000
17110 2200000000
17167 1150000000
17167 150000000000
17172 150
17189 93939100
17329 7424520
17382 479000000
17389 605000000
17458 341000000000
17502 66300000
17505 36700000000
17567 168000000
17567 385000000
17629 50900000
17683 17600000
17715 34900000
17802 3000000000
17815 285000000
17900 2470000
17928 91600
17941 1490000000
17950 37065600
17990 2560000
18045 1500000000
18045 1500000000
18047 4000000
18145 19400000
18156 304000
18156 9100000000
18156 56800000000
18171 7600000
18184 854000000
18192 10400000000
18192 40500000000
18199 202000000000
18008 13000000000
18057 67000000000
18414 300000000
18276 100000000
18289 112000000000
18301 2543730000
18305 15700000000
18334 270000000
18380 314000000000
18381 1780000000
18430 8910000000
18430 33000000000
18443 13300000000
18443 26000000000
18533 12800000000
18557 434000000
18589 124000000
18597 1800000000
18627 2000000000
18779 1100000000
18779 7100000000
18632 10500000000
18632 47000000000
18638 82200000000
18687 212000000000
18707 7900000000
18742 58300000000
18748 15000000000
18751 73700000000
18772 63000000000
18773 26800000000
18773 24100000
18786 3400000000
18789 1600000
18789 215000000000
18813 2350000
18835 5540000000
18837 4420000000
18850 370000000000
18908 5530000000
18911 1350000000000
18941 410000000000
18969 631000000000
19012 355000000000
19430 21000000000000
};
\addplot [draw=red, fill=red, mark=*, only marks]
table{%
x  y
17683 17600000
17941 1490000000
18380 314000000000
19430 21000000000000
};
\end{axis}

\end{tikzpicture}


==> plot.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Publication Date},
xmin=14410, xmax=19830,
xtick style={color=black},
xtick={13879,14610,15340,16071,16801,17532,18262,18993,19723},
xticklabels={2008,2010,2012,2014,2016,2018,2020,2022,2024},
y grid style={darkgray176},
ylabel={Training compute (Terraflop)},
ymin=36.059848328477, ymax=76289838352633.9,
ymode=log,
ytick style={color=black},
ytick={0.1,10,1000,100000,10000000,1000000000,100000000000,10000000000000,1e+15,1e+17},
yticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{9}}\),
  \(\displaystyle {10^{11}}\),
  \(\displaystyle {10^{13}}\),
  \(\displaystyle {10^{15}}\),
  \(\displaystyle {10^{17}}\)
}
]
\addplot [draw=black, fill=black, mark=*, only marks]
table{%
x  y
14410 1000
14669 131
14742 350
14878 3410
14878 61400
15383 3730
15494 6040
15613 470000
15706 2300
15970 137000
15994 38900
16021 532000
16044 1340930
16059 475.2
16231 518000
16239 6110000
16314 1560000
16317 8524000
16323 7300000
16426 60500
16472 24000000
16593 1560000
16687 380000000
16777 26000000
16779 12100000
16827 1900000000
16973 61492.9
17003 145411
17003 96940.8
17070 6900000000
17081 44000000
17110 2200000000
17167 1150000000
17167 150000000000
17172 150
17189 93939100
17329 7424520
17382 479000000
17389 605000000
17458 341000000000
17502 66300000
17505 36700000000
17567 168000000
17567 385000000
17629 50900000
17683 17600000
17715 34900000
17802 3000000000
17815 285000000
17900 2470000
17928 91600
17941 1490000000
17950 37065600
17990 2560000
18045 1500000000
18045 1500000000
18047 4000000
18145 19400000
18156 304000
18156 9100000000
18156 56800000000
18171 7600000
18184 854000000
18192 10400000000
18192 40500000000
18199 202000000000
18008 13000000000
18057 67000000000
18414 300000000
18276 100000000
18289 112000000000
18301 2543730000
18305 15700000000
18334 270000000
18380 314000000000
18381 1780000000
18430 8910000000
18430 33000000000
18443 13300000000
18443 26000000000
18533 12800000000
18557 434000000
18589 124000000
18597 1800000000
18627 2000000000
18779 1100000000
18779 7100000000
18632 10500000000
18632 47000000000
18638 82200000000
18687 212000000000
18707 7900000000
18742 58300000000
18748 15000000000
18751 73700000000
18772 63000000000
18773 26800000000
18773 24100000
18786 3400000000
18789 1600000
18789 215000000000
18813 2350000
18835 5540000000
18837 4420000000
18850 370000000000
18908 5530000000
18911 1350000000000
18941 410000000000
18969 631000000000
19012 355000000000
19430 21000000000000
};
\addplot [draw=red, fill=red, mark=*, only marks]
table{%
x  y
17683 17600000
17941 1490000000
18380 314000000000
19430 21000000000000
};
\end{axis}

\end{tikzpicture}

